Astronomy outreach in Namibia: H.E.S.S. and beyond

Astronomy plays a major role in the scientific landscape of Namibia. Because of its excellent sky conditions, Namibia is home to ground-based observatories like the High Energy Spectroscopic System (H.E.S.S.), in operation since 2002. Located near the Gamsberg mountain, H.E.S.S. performs groundbreaking science by detecting very-high-energy gamma rays from astronomical objects. The fascinating stories behind many of them are featured regularly in the ``Source of the Month'', a blog-like format intended for the general public with more than 170 features to date. In addition to other online communication via social media, H.E.S.S. outreach activities have been covered locally, e.g. through `open days' and guided tours on the H.E.S.S. site itself. An overview of the H.E.S.S. outreach activities are presented in this contribution, along with discussions relating to the current landscape of astronomy outreach and education in Namibia. There has also been significant activity in the country in recent months, whereby astronomy is being used to further sustainable development via human capacity-building. Finally, as we take into account the future prospects of radio astronomy in the country, momentum for a wider range of astrophysics research is clearly building -- this presents a great opportunity for the astronomy community to come together to capitalise on this movement and support astronomy outreach, with the overarching aim to advance sustainable development in Namibia.

==> authors_ALL_ICRC.tex <==
\scriptsize
\noindent
H.~Abdalla$^{1}$, 
F.~Aharonian$^{2,3,4}$, 
F.~Ait~Benkhali$^{3}$, 
E.O.~Ang\"uner$^{5}$, 
C.~Arcaro$^{6}$, 
C.~Armand$^{7}$, 
T.~Armstrong$^{8}$, 
H.~Ashkar$^{9}$, 
M.~Backes$^{1,6}$, 
V.~Baghmanyan$^{10}$, 
V.~Barbosa~Martins$^{11}$, 
A.~Barnacka$^{12}$, 
M.~Barnard$^{6}$, 
R.~Batzofin$^{13}$, 
Y.~Becherini$^{14}$, 
D.~Berge$^{11}$, 
K.~Bernl\"ohr$^{3}$, 
B.~Bi$^{15}$, 
M.~B\"ottcher$^{6}$, 
C.~Boisson$^{16}$, 
J.~Bolmont$^{17}$, 
M.~de~Bony~de~Lavergne$^{7}$, 
M.~Breuhaus$^{3}$, 
R.~Brose$^{2}$, 
F.~Brun$^{9}$, 
T.~Bulik$^{18}$, 
T.~Bylund$^{14}$, 
F.~Cangemi$^{17}$, 
S.~Caroff$^{17}$, 
S.~Casanova$^{10}$, 
J.~Catalano$^{19}$, 
P.~Chambery$^{20}$, 
T.~Chand$^{6}$, 
A.~Chen$^{13}$, 
G.~Cotter$^{8}$, 
M.~Cury{\l}o$^{18}$, 
H.~Dalgleish$^{1,8}$, 
J.~Damascene~Mbarubucyeye$^{11}$, 
I.D.~Davids$^{1}$, 
J.~Davies$^{8}$, 
J.~Devin$^{20}$, 
A.~Djannati-Ata\"i$^{21}$, 
A.~Dmytriiev$^{16}$, 
A.~Donath$^{3}$, 
V.~Doroshenko$^{15}$, 
L.~Dreyer$^{6}$, 
L.~Du~Plessis$^{6}$, 
C.~Duffy$^{22}$, 
K.~Egberts$^{23}$, 
S.~Einecke$^{24}$, 
J.-P.~Ernenwein$^{5}$, 
S.~Fegan$^{25}$, 
K.~Feijen$^{24}$, 
A.~Fiasson$^{7}$, 
G.~Fichet~de~Clairfontaine$^{16}$, 
G.~Fontaine$^{25}$, 
F.~Lott$^{1}$, 
M.~F\"u{\ss}ling$^{11}$, 
S.~Funk$^{19}$, 
S.~Gabici$^{21}$, 
Y.A.~Gallant$^{26}$, 
G.~Giavitto$^{11}$, 
L.~Giunti$^{21,9}$, 
D.~Glawion$^{19}$, 
J.F.~Glicenstein$^{9}$, 
M.-H.~Grondin$^{20}$, 
S.~Hattingh$^{6}$, 
M.~Haupt$^{11}$, 
G.~Hermann$^{3}$, 
J.A.~Hinton$^{3}$, 
W.~Hofmann$^{3}$, 
C.~Hoischen$^{23}$, 
T.~L.~Holch$^{11}$, 
M.~Holler$^{27}$, 
D.~Horns$^{28}$, 
Zhiqiu~Huang$^{3}$, 
D.~Huber$^{27}$, 
M.~H\"{o}rbe$^{8}$, 
M.~Jamrozy$^{12}$, 
F.~Jankowsky$^{29}$, 
V.~Joshi$^{19}$, 
I.~Jung-Richardt$^{19}$, 
E.~Kasai$^{1}$, 
K.~Katarzy{\'n}ski$^{30}$, 
U.~Katz$^{19}$, 
D.~Khangulyan$^{31}$, 
B.~Kh\'elifi$^{21}$, 
S.~Klepser$^{11}$, 
W.~Klu\'{z}niak$^{32}$, 
Nu.~Komin$^{13}$, 
R.~Konno$^{11}$, 
K.~Kosack$^{9}$, 
D.~Kostunin$^{11}$, 
M.~Kreter$^{6}$, 
G.~Kukec~Mezek$^{14}$, 
A.~Kundu$^{6}$, 
G.~Lamanna$^{7}$, 
S.~Le Stum$^{5}$, 
A.~Lemi\`ere$^{21}$, 
M.~Lemoine-Goumard$^{20}$, 
J.-P.~Lenain$^{17}$, 
F.~Leuschner$^{15}$, 
C.~Levy$^{17}$, 
T.~Lohse$^{33}$, 
A.~Luashvili$^{16}$, 
I.~Lypova$^{29}$, 
J.~Mackey$^{2}$, 
J.~Majumdar$^{11}$, 
D.~Malyshev$^{15}$, 
D.~Malyshev$^{19}$, 
V.~Marandon$^{3}$, 
P.~Marchegiani$^{13}$, 
A.~Marcowith$^{26}$, 
A.~Mares$^{20}$, 
G.~Mart\'i-Devesa$^{27}$, 
R.~Marx$^{29}$, 
G.~Maurin$^{7}$, 
P.J.~Meintjes$^{34}$, 
M.~Meyer$^{19}$, 
A.~Mitchell$^{3}$, 
R.~Moderski$^{32}$, 
L.~Mohrmann$^{19}$, 
A.~Montanari$^{9}$, 
C.~Moore$^{22}$, 
P.~Morris$^{8}$, 
E.~Moulin$^{9}$, 
J.~Muller$^{25}$, 
T.~Murach$^{11}$, 
K.~Nakashima$^{19}$, 
M.~de~Naurois$^{25}$, 
A.~Nayerhoda$^{10}$, 
H.~Ndiyavala$^{6}$, 
J.~Niemiec$^{10}$, 
A.~Priyana~Noel$^{12}$, 
P.~O'Brien$^{22}$, 
L.~Oberholzer$^{6}$, 
S.~Ohm$^{11}$, 
L.~Olivera-Nieto$^{3}$, 
E.~de~Ona~Wilhelmi$^{11}$, 
M.~Ostrowski$^{12}$, 
S.~Panny$^{27}$, 
M.~Panter$^{3}$, 
R.D.~Parsons$^{33}$, 
G.~Peron$^{3}$, 
S.~Pita$^{21}$, 
V.~Poireau$^{7}$, 
D.A.~Prokhorov$^{35}$, 
H.~Prokoph$^{11}$, 
G.~P\"uhlhofer$^{15}$, 
M.~Punch$^{21,14}$, 
A.~Quirrenbach$^{29}$, 
P.~Reichherzer$^{9}$, 
A.~Reimer$^{27}$, 
O.~Reimer$^{27}$, 
Q.~Remy$^{3}$, 
M.~Renaud$^{26}$, 
B.~Reville$^{3}$, 
F.~Rieger$^{3}$, 
C.~Romoli$^{3}$, 
G.~Rowell$^{24}$, 
B.~Rudak$^{32}$, 
H.~Rueda Ricarte$^{9}$, 
E.~Ruiz-Velasco$^{3}$, 
V.~Sahakian$^{36}$, 
S.~Sailer$^{3}$, 
H.~Salzmann$^{15}$, 
D.A.~Sanchez$^{7}$, 
A.~Santangelo$^{15}$, 
M.~Sasaki$^{19}$, 
J.~Sch\"afer$^{19}$, 
H.M.~Schutte$^{6}$, 
U.~Schwanke$^{33}$, 
F.~Sch\"ussler$^{9}$, 
M.~Senniappan$^{14}$, 
A.S.~Seyffert$^{6}$, 
J.N.S.~Shapopi$^{1}$, 
K.~Shiningayamwe$^{1}$, 
R.~Simoni$^{35}$, 
A.~Sinha$^{26}$, 
H.~Sol$^{16}$, 
H.~Spackman$^{8}$, 
A.~Specovius$^{19}$, 
S.~Spencer$^{8}$, 
M.~Spir-Jacob$^{21}$, 
{\L.}~Stawarz$^{12}$, 
R.~Steenkamp$^{1}$, 
C.~Stegmann$^{23,11}$, 
S.~Steinmassl$^{3}$, 
C.~Steppa$^{23}$, 
L.~Sun$^{35}$, 
T.~Takahashi$^{37}$, 
T.~Tanaka$^{38}$, 
T.~Tavernier$^{9}$, 
A.M.~Taylor$^{11}$, 
R.~Terrier$^{21}$, 
J.~H.E.~Thiersen$^{6}$, 
C.~Thorpe-Morgan$^{15}$, 
M.~Tluczykont$^{28}$, 
L.~Tomankova$^{19}$, 
M.~Tsirou$^{3}$, 
N.~Tsuji$^{39}$, 
R.~Tuffs$^{3}$, 
Y.~Uchiyama$^{31}$, 
D.J.~van~der~Walt$^{6}$, 
C.~van~Eldik$^{19}$, 
C.~van~Rensburg$^{1}$, 
B.~van~Soelen$^{34}$, 
G.~Vasileiadis$^{26}$, 
J.~Veh$^{19}$, 
C.~Venter$^{6}$, 
P.~Vincent$^{17}$, 
J.~Vink$^{35}$, 
H.J.~V\"olk$^{3}$, 
S.J.~Wagner$^{29}$, 
J.~Watson$^{8}$, 
F.~Werner$^{3}$, 
R.~White$^{3}$, 
A.~Wierzcholska$^{10}$, 
Yu~Wun~Wong$^{19}$, 
H.~Yassin$^{6}$, 
A.~Yusafzai$^{19}$, 
M.~Zacharias$^{16}$, 
R.~Zanin$^{3}$, 
D.~Zargaryan$^{2,4}$, 
A.A.~Zdziarski$^{32}$, 
A.~Zech$^{16}$, 
S.J.~Zhu$^{11}$, 
A.~Zmija$^{19}$, 
S.~Zouari$^{21}$ and 
N.~\.Zywucka$^{6}$.

\medskip


\noindent
$^{1}$University of Namibia, Department of Physics, Private Bag 13301, Windhoek 10005, Namibia\\
$^{2}$Dublin Institute for Advanced Studies, 31 Fitzwilliam Place, Dublin 2, Ireland\\
$^{3}$Max-Planck-Institut f\"ur Kernphysik, P.O. Box 103980, D 69029 Heidelberg, Germany\\
$^{4}$High Energy Astrophysics Laboratory, RAU,  123 Hovsep Emin St  Yerevan 0051, Armenia\\
$^{5}$Aix Marseille Universit\'e, CNRS/IN2P3, CPPM, Marseille, France\\
$^{6}$Centre for Space Research, North-West University, Potchefstroom 2520, South Africa\\
$^{7}$Laboratoire d'Annecy de Physique des Particules, Univ. Grenoble Alpes, Univ. Savoie Mont Blanc, CNRS, LAPP, 74000 Annecy, France\\
$^{8}$University of Oxford, Department of Physics, Denys Wilkinson Building, Keble Road, Oxford OX1 3RH, UK\\
$^{9}$IRFU, CEA, Universit\'e Paris-Saclay, F-91191 Gif-sur-Yvette, France\\
$^{10}$Instytut Fizyki J\c{a}drowej PAN, ul. Radzikowskiego 152, 31-342 Krak{\'o}w, Poland\\
$^{11}$DESY, D-15738 Zeuthen, Germany\\
$^{12}$Obserwatorium Astronomiczne, Uniwersytet Jagiello{\'n}ski, ul. Orla 171, 30-244 Krak{\'o}w, Poland\\
$^{13}$School of Physics, University of the Witwatersrand, 1 Jan Smuts Avenue, Braamfontein, Johannesburg, 2050 South Africa\\
$^{14}$Department of Physics and Electrical Engineering, Linnaeus University,  351 95 V\"axj\"o, Sweden\\
$^{15}$Institut f\"ur Astronomie und Astrophysik, Universit\"at T\"ubingen, Sand 1, D 72076 T\"ubingen, Germany\\
$^{16}$Laboratoire Univers et Théories, Observatoire de Paris, Université PSL, CNRS, Université de Paris, 92190 Meudon, France\\
$^{17}$Sorbonne Universit\'e, Universit\'e Paris Diderot, Sorbonne Paris Cit\'e, CNRS/IN2P3, Laboratoire de Physique Nucl\'eaire et de Hautes Energies, LPNHE, 4 Place Jussieu, F-75252 Paris, France\\
$^{18}$Astronomical Observatory, The University of Warsaw, Al. Ujazdowskie 4, 00-478 Warsaw, Poland\\
$^{19}$Friedrich-Alexander-Universit\"at Erlangen-N\"urnberg, Erlangen Centre for Astroparticle Physics, Erwin-Rommel-Str. 1, D 91058 Erlangen, Germany\\
$^{20}$Universit\'e Bordeaux, CNRS/IN2P3, Centre d'\'Etudes Nucl\'eaires de Bordeaux Gradignan, 33175 Gradignan, France\\
$^{21}$Université de Paris, CNRS, Astroparticule et Cosmologie, F-75013 Paris, France\\
$^{22}$Department of Physics and Astronomy, The University of Leicester, University Road, Leicester, LE1 7RH, United Kingdom\\
$^{23}$Institut f\"ur Physik und Astronomie, Universit\"at Potsdam,  Karl-Liebknecht-Strasse 24/25, D 14476 Potsdam, Germany\\
$^{24}$School of Physical Sciences, University of Adelaide, Adelaide 5005, Australia\\
$^{25}$Laboratoire Leprince-Ringuet, École Polytechnique, CNRS, Institut Polytechnique de Paris, F-91128 Palaiseau, France\\
$^{26}$Laboratoire Univers et Particules de Montpellier, Universit\'e Montpellier, CNRS/IN2P3,  CC 72, Place Eug\`ene Bataillon, F-34095 Montpellier Cedex 5, France\\
$^{27}$Institut f\"ur Astro- und Teilchenphysik, Leopold-Franzens-Universit\"at Innsbruck, A-6020 Innsbruck, Austria\\
$^{28}$Universit\"at Hamburg, Institut f\"ur Experimentalphysik, Luruper Chaussee 149, D 22761 Hamburg, Germany\\
$^{29}$Landessternwarte, Universit\"at Heidelberg, K\"onigstuhl, D 69117 Heidelberg, Germany\\
$^{30}$Institute of Astronomy, Faculty of Physics, Astronomy and Informatics, Nicolaus Copernicus University,  Grudziadzka 5, 87-100 Torun, Poland\\
$^{31}$Department of Physics, Rikkyo University, 3-34-1 Nishi-Ikebukuro, Toshima-ku, Tokyo 171-8501, Japan\\
$^{32}$Nicolaus Copernicus Astronomical Center, Polish Academy of Sciences, ul. Bartycka 18, 00-716 Warsaw, Poland\\
$^{33}$Institut f\"ur Physik, Humboldt-Universit\"at zu Berlin, Newtonstr. 15, D 12489 Berlin, Germany\\
$^{34}$Department of Physics, University of the Free State,  PO Box 339, Bloemfontein 9300, South Africa\\
$^{35}$GRAPPA, Anton Pannekoek Institute for Astronomy, University of Amsterdam,  Science Park 904, 1098 XH Amsterdam, The Netherlands\\
$^{36}$Yerevan Physics Institute, 2 Alikhanian Brothers St., 375036 Yerevan, Armenia\\
$^{37}$Kavli Institute for the Physics and Mathematics of the Universe (WPI), The University of Tokyo Institutes for Advanced Study (UTIAS), The University of Tokyo, 5-1-5 Kashiwa-no-Ha, Kashiwa, Chiba, 277-8583, Japan\\
$^{38}$Department of Physics, Konan University, 8-9-1 Okamoto, Higashinada, Kobe, Hyogo 658-8501, Japan\\
$^{39}$RIKEN, 2-1 Hirosawa, Wako, Saitama 351-0198, Japan\\

